Probing the chiral limit with clover fermions II: The baryon sector

Algorithmic progress in recent years made it possible to simulate QCD with Nf=2 flavours of O(a)-improved Wilson fermions at very light quark masses. We present the current results for baryon spectrum states, the nucleon axial coupling and the lowest moment of unpolarised nucleon structure functions. Special emphasis is given to a comparison of our calculations with results from chiral effective theories.

==> figs/Makefile <==
STEM =	r0 fitMnBchpt fitMdeltaChpt1 var-r0 fitGaBchpt-beta-r0c \
	x-umd x-upd
EPS  =	$(STEM:%=%.eps) 
PDF  =	$(STEM:%=%.pdf)

all:	$(EPS) $(PDF)

%.eps:  %.agr
	gracebat -hardcopy -hdevice PostScript -printfile - $*.agr > $*.ps && \
	ps2epsi $*.ps $*.eps

%.pdf:	%.eps
	epstopdf --outfile=$@ $<

